Fast IR Drop Estimation with Machine Learning

IR drop constraint is a fundamental requirement enforced in almost all chip designs. However, its evaluation takes a long time, and mitigation techniques for fixing violations may require numerous iterations. As such, fast and accurate IR drop prediction becomes critical for reducing design turnaround time. Recently, machine learning (ML) techniques have been actively studied for fast IR drop estimation due to their promise and success in many fields. These studies target at various design stages with different emphasis, and accordingly, different ML algorithms are adopted and customized. This paper provides a review to the latest progress in ML-based IR drop estimation techniques. It also serves as a vehicle for discussing some general challenges faced by ML applications in electronics design automation (EDA), and demonstrating how to integrate ML models with conventional techniques for the better efficiency of EDA tools.

==> _txt/1_background.tex <==

\iffalse

\vspace{-2mm}
\section{Background}
\label{sec:background}


\subsection{Vectors in Dynamic IR Drop}

The requirement on switching activity is a limitation of the dynamic IR drop, considering the late availability of switching activities in many design processes. Such activity is also referred as switching vector or simulation pattern. There are two options for dynamic IR drop analysis: (1) vector-based analysis with switching vectors. (2) vectorless analysis by propagated switching probability. %The second option bypasses .



Figure \ref{static} shows the difference between static and dynamic IR drop under different clock frequencies \cite{nithin2010dynamic}. The dynamic IR drop is decided by the highest transient dynamic current, which is less dependent on the clock period. The dynamic IR drop is a more strict constraint and more difficult to predict \cite{lin2004full, nithin2010dynamic}.

Static IR drop is commonly used to validate the robustness of PDN, especially on old technology nodes, where sufficient natural decoupling capacitance is available ~\cite{Cadence, nithin2010dynamic}. Since it does not require switching activity as input, it is applied at early design stage when simulation pattern is not yet available.

In contrast with static IR drop, dynamic IR drop considers switching activities during analysis. The dynamic IR drop is analyzed either using vectorless analysis or vector-based analysis. The vectorless analysis usually simulates IR drop by propagating switching probability, while vector-based IR drop relies on switching patterns. One limitation of vector-based dynamic IR drop is its reliance on switching activities, which is usually not available at early design stages~\cite{nithin2010dynamic, xie2020powernet}.


\subsection{Power Delivery Network}
Power is distributed across the chip through power delivery network (PDN).  The metal lines on PDN are also referred to as power grids, power straps or power stripes. As technology node shrinks, wires get thinner with higher resistance per unit length, but the total power consumption is not reduced. This exaggerates voltage drop when current flow through the power straps. Thus IR drop is one of the key constraints on PDN design and optimization, and excessive IR drop can be mitigated by enhancing the PDN on those hotspot regions. However, overdesigned PDN consumes extra routing resources, which may violate the routability constraint.  There has been many traditional methods on power grids analysis \cite{zhao2002hierarchical, qian2005power, chen2001efficient, zhuo2008power, su2003power}. Most of them find a faster solution to the well-known equation (\ref{equ}) in power grid analysis, where G is the conductance matrix, v is the desired vector of node voltages, and u is a vector of voltage and current source.

\begin{equation}
\vspace{-3mm}
Gv = u
\label{equ}
\end{equation}
\fi


\iffalse

\subsection{Representative ML Algorithms}

The representative ML algorithms that are frequently used for IR drop estimation include artificial neural network (ANN), XGBoost \cite{chen2016xgboost}, and convolutional neural network (CNN) \cite{krizhevsky2012imagenet}. ANN and XGBoost typically process one-dimensional inputs, while CNN handles two-dimensional features.

ANN is also referred to as multilayer perceptron (MLP). XGBoost is a very efficient and popular implementation of gradient boosting decision tree (GDBT) \cite{friedman2001greedy}. The GBRT builds decision trees sequentially, with each tree built on the error of the previous ones. CNN has generated huge impact from image classification to video processing. A typical structure of CNN is composed by convolutional layers, pooling layers and fully-connected layers. Convolutional layers and pooling layers perform downsampling and produce a feature map smaller than the input. The fully connected layers at the end of CNN generate the final output.

\fi

==> _txt/3_static.tex <==


